Flexible and scalable privacy assessment for very large datasets, with an application to official governmental microdata

We present a systematic refactoring of the conventional treatment of privacy analyses, basing it on mathematical concepts from the framework of Quantitative Information Flow (QIF). The approach we suggest brings three principal advantages: it is flexible, allowing for precise quantification and comparison of privacy risks for attacks both known and novel; it can be computationally tractable for very large, longitudinal datasets; and its results are explainable both to politicians and to the general public. We apply our approach to a very large case study: the Educational Censuses of Brazil, curated by the governmental agency INEP, which comprise over 90 attributes of approximately 50 million individuals released longitudinally every year since 2007. These datasets have only very recently (2018-2021) attracted legislation to regulate their privacy -- while at the same time continuing to maintain the openness that had been sought in Brazilian society. INEP's reaction to that legislation was the genesis of our project with them. In our conclusions here we share the scientific, technical, and communication lessons we learned in the process.

==> Makefile <==
all:
	./compile all
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe  

draft:
	./compile draft
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe  

bleck:
	./compile bleck
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe  

print:
	./compile print
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe  

review:
	./compile review
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe   

clean:
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe  

reset:
	./compile reset
	@rm -f \
		*.aux **/*.aux \
		*.log **/*.log \
		*.bbl **/*.bbl \
		*.blg **/*.blg \
		*.toc **/*.toc \
		*.out **/*.out \
		*.idx **/*.idx \
		*.spl **/*.spl \
		*.lof **/*.lof \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.synctex.gz **/*.synctex.gz \
		*.ent **/*.ent \
		*.glo **/*.glo \
		*.glsdefs **/*.glsdefs \
		*.ist **/*.ist \
		*.lot **/*.lot \
		*.brf **/*.brf \
		*.acn **/*.acn 
	@rm -f \
		*.cpt **/*.cpt \
		*.loe **/*.loe  


==> compile <==
#!/bin/bash

# Move to the correct directory, so this can be clicked from anywhere.
cd "`dirname \"$0\"`"

# Main file
filename="main"

# Output name
outputname="main"

# Suffixes for different file versions.
strdraft="[draft]"
strprint="[print]"
strreview="[review]"

# Checks if any string has been passed as a parameter.
if [ $# -ne 0 ]; 
then
	case "$1" in
		all) 
			draftmode=true;
			bleckmode=true;
			reviewmode=true;
			reset=false;
			echo "You have passed argument '$1'.";
			echo "I will produce all the DRAFT and BLECK/PRINT and REVIEW versions of the pdf."
			;;
		draft) 
			draftmode=true;
			bleckmode=false;
			reviewmode=false;
			reset=false;
			echo "You have passed argument '$1'.";
			echo "I will produce only the DRAFT version of the pdf."
			;;
		bleck) 
			draftmode=false;
			bleckmode=true;
			reviewmode=false;
			reset=false;
			echo "You have passed argument '$1'.";
			echo "I will produce only the BLECK/PRINT version of the pdf."
			;;
		print) 
			draftmode=false;
			bleckmode=true;
			reviewmode=false;
			reset=false;
			echo "You have passed argument '$1'.";
			echo "I will produce only the BLECK/PRINT version of the pdf."
			;;
		review) 
			draftmode=false;
			bleckmode=false;
			reviewmode=true;
			reset=false;
			echo "You have passed argument '$1'.";
			echo "I will produce only the REVIEW version of the pdf."
			;;
		reset)
			draftmode=false;
			bleckmode=false;
			reviewmode=false;
			reset=true;
			echo "You have passed argument '$1'.";
			echo "I will just erase the following files: \""$outputname".pdf\", \""$outputname$strdraft".pdf\" and \""$outputname$strprint".pdf\""
			;; 
		*) 
			draftmode=false;
			bleckmode=false;
			reviewmode=false;
			reset=false;
			echo "You have passed an invalid argument '$1'.";
			echo "I won't do anything"
		;;
	esac
else
	draftmode=true;
	bleckmode=true;
	reviewmode=false;
	echo "You haven't passed any argument.";
	echo "I will produce both the DRAFT and BLECK/PRINT versions of the pdf, but not the REVIEW mode."
fi

if [ "$draftmode" = true ]; 
then 
	echo "I am now producing the DRAFT version of the pdf..."
	# Generates draft mode version of pdf
	pdflatex -jobname="$outputname$strdraft" "\def\ForceDraft{} \input{$filename}"
	for auxfile in *.aux
	do
		bibtex $auxfile
	done
	pdflatex -jobname="$outputname$strdraft" "\def\ForceDraft{} \input{$filename}"
	pdflatex -jobname="$outputname$strdraft" "\def\ForceDraft{} \input{$filename}"
fi

if [ "$bleckmode" = true ];
then 
	echo "I am now producing the BLECK/PRINT version of the pdf..."
	# Generates draft mode version of pdf
	pdflatex -jobname="$outputname$strprint" "\def\ForceBleck{} \input{$filename}"
	for auxfile in *.aux
	do
		bibtex $auxfile
	done
	pdflatex -jobname="$outputname$strprint" "\def\ForceBleck{} \input{$filename}"
	pdflatex -jobname="$outputname$strprint" "\def\ForceBleck{} \input{$filename}"
fi

if [ "$reviewmode" = true ];
then 
	echo "I am now producing the REVIEW version of the pdf..."
	# Generates review mode version of pdf
	pdflatex -jobname="$outputname$strreview" "\def\ForceReview{} \input{$filename}"
	for auxfile in *.aux
	do
		bibtex $auxfile
	done
	pdflatex -jobname="$outputname$strreview" "\def\ForceReview{} \input{$filename}"
	pdflatex -jobname="$outputname$strreview" "\def\ForceReview{} \input{$filename}"
fi

if [ "$reset" = true ];
then 
	echo "I am now erasing the following files: \""$outputname".pdf\", \""$outputname$strdraft".pdf\" and \""$outputname$strprint".pdf\" and \""$outputname$strreview".pdf\"..."
	rm -f "$outputname"".pdf"
	rm -f "$outputname$strdraft"".pdf"
	rm -f "$outputname$strprint"".pdf"
	rm -f "$outputname$strreview"".pdf"
fi

echo; echo "All done! Press return."
read Z

